CTGAN: Semantic-guided Conditional Texture Generator for 3D Shapes

The entertainment industry relies on 3D visual content to create immersive experiences, but traditional methods for creating textured 3D models can be time-consuming and subjective. Generative networks such as StyleGAN have advanced image synthesis, but generating 3D objects with high-fidelity textures is still not well explored, and existing methods have limitations. We propose the Semantic-guided Conditional Texture Generator (CTGAN), producing high-quality textures for 3D shapes that are consistent with the viewing angle while respecting shape semantics. CTGAN utilizes the disentangled nature of StyleGAN to finely manipulate the input latent codes, enabling explicit control over both the style and structure of the generated textures. A coarse-to-fine encoder architecture is introduced to enhance control over the structure of the resulting textures via input segmentation. Experimental results show that CTGAN outperforms existing methods on multiple quality metrics and achieves state-of-the-art performance on texture generation in both conditional and unconditional settings.

==> Figure/fig_example.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/qualitative_result_1.png}
    \caption{The Qualitative comparison with existing methods.}
    \label{fig:qualitative_result_1.png}
\end{figure}

==> Figure/fig_face_result_condition.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/face_result_condition.png}
    \caption{The Qualitative comparison with existing methods.}
    \label{fig:qualitative_result_face_1}
\end{figure}


==> Figure/fig_face_result_uncondition.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/face_result_uncondition.png}
    \caption{The Qualitative comparison with existing methods.}
    \label{fig:qualitative_result_face_2}
\end{figure}


==> Figure/fig_our_mixture.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/mixing_new.png}
    \caption{The Qualitative comparison with existing methods.}
    \label{fig:our_mixture}
\end{figure}


==> Figure/fig_our_mixture_1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/our_mixing_1.png}
    \caption{The Qualitative comparison with existing methods.}
    \label{fig:our_mixture_1}
\end{figure}


==> Figure/fig_our_mixture_2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/our_mixing_2.png}
    \caption{The Qualitative comparison with existing methods.}
    \label{fig:our_mixture_2}
\end{figure}


==> Figure/fig_qualitative_result2.tex <==
\begin{figure*}
    \flushleft
    \includegraphics[width=\textwidth]{Figure/images/result_uncondition_v2.png}
    \caption{\tb{Qualitative comparison under unconditional setting.} First row: the input 3D models. Bottom 3 rows (cars part): three different randomly selected texture maps of the given 3D models from the first row for each method.
    %
    Bottom 3 rows (faces part): two different views of the generated 3D textured models for each method using and 3D models from the first row.
    %
    Our method produce better texture maps that align well with the input 3D model and are more diverse.}
    \label{fig:qualitative_result_2}
\end{figure*}

==> Figure/fig_segmentation_result.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figure/images/input_seg_num.png}
%     \caption{Different class number of segmentation label.}
%     \label{fig:input_seg_num}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/different_seg_num_result.png}
    \caption{\tb{Qualitative comparisons with different class numbers.} We visualize the difference of the generated front-view texture maps across different class numbers (10, 14, and 32).
    The results get worse as we increase the number of the classes due to insufficient supervision for fine-grained class labels.
    }
    \label{fig:different_seg_num_result}
\end{figure}

==> Figure/fig_style_manipute_mix.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/mixture_styleGAN2.png}
    \caption{Swap the last six layers of style codes in B from A.}
    \label{fig:styleGAN2_mixture}
\end{figure}

==> Figure/fig_sup_result.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 22.png}
    \label{fig:sup_result_1}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 1.png}
    \label{fig:sup_result_1}
\end{figure}
\clearpage

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 24.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 20.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 32.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 30.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 8.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 2.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 12.png}
    \label{fig:sup_result_1}
\end{figure} \clearpage


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/sup_images/Frame 4.png}
%     \label{fig:sup_result_1}
% \end{figure} \clearpage


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/sup_images/Frame 17.png}
%     \label{fig:sup_result_1}
% \end{figure} \clearpage

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/sup_images/Frame 29.png}
%     \label{fig:sup_result_1}
% \end{figure} \clearpage



\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/sup_images/Frame 21.png}
    \label{fig:sup_result_1}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/sup_images/Frame 16.png}
%     \label{fig:sup_result_1}
% \end{figure} \clearpage

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/sup_images/Frame 3.png}
%     \label{fig:sup_result_1}
% \end{figure} \clearpage

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/sup_images/Frame 19.png}
%     \label{fig:sup_result_1}
% \end{figure} \clearpage


==> Figure/fig_teaser.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.55\textwidth]{Figure/images/teaser.png}
%     \captionof{figure}{\tb{Conditional Texture Generation}. We propose a new conditional texture generator (CTGAN) that is conditioned on the 3D model (a) and style images (b) and is able to generate high-quality texture maps (c) for 3D objects. Our textured 3D models (d) are view consistent and aligned with the input style images.}
%     \label{fig:teaser}
% \end{figure*}

\begin{center}
    \centering
    % \hspace*{-8.3cm}
    \includegraphics[width=\textwidth]{Figure/images/teaser_v3.png}
    % \vspace{0.5mm}
    \captionof{figure}{\tb{Conditional texture generation}. We propose a new conditional texture generator (CTGAN) that is conditioned on the segmentation map derived from the 3D model (a) and style images (b) and is able to generate high-quality texture maps (c) for 3D objects. Our textured 3D models (d) are view consistent and aligned with the input style images.}
    \label{fig:teaser}
\end{center}


% \begin{figure*}[ht]
% \begin{overpic}[width=\textwidth]{figure/images/archit_v6.png}
% \put(1, 41){\begin{minipage}{0.15\textwidth}\centering Object Detection\\(\secref{objectdetection}) \end{minipage}}
% \put(1.5, 21){\begin{minipage}{0.1\textwidth}\centering $\{\instngray\}_{i=1}^N$ \end{minipage}}
% \put(2, 1.5){\begin{minipage}{0.1\textwidth}\centering $\instnboxi$ \end{minipage}}
% \put(21.5, 23.5){\begin{minipage}{0.1\textwidth}\centering $\instngray$ \end{minipage}}
% \put(19.5, 1.5){\begin{minipage}{0.1\textwidth}\centering Input $\grayimg$ \end{minipage}}
% \put(38, 41){\begin{minipage}{0.2\textwidth}\centering Instance Colorization\\(\secref{backbone}) \end{minipage}}
% \put(36, 21.5){\begin{minipage}{0.25\textwidth}\centering Fusion Module (\secref{fusionmodule}) \end{minipage}}
% \put(38, 2){\begin{minipage}{0.2\textwidth}\centering (\secref{backbone})\\Full-image Colorization \end{minipage}}
% \put(65, 23.5){\begin{minipage}{0.1\textwidth}\centering $\instnpred$ \end{minipage}}
% \put(87, 23.5){\begin{minipage}{0.1\textwidth}\centering $\instnGT$ \end{minipage}}
% \put(65, 1.5){\begin{minipage}{0.1\textwidth}\centering $\predimg$ \end{minipage}}
% \put(87, 1.5){\begin{minipage}{0.1\textwidth}\centering $\predGT$ \end{minipage}}
% \put(75.5, 30.5){\begin{minipage}{0.1\textwidth}\centering loss \end{minipage}}
% \put(75.5, 8.5){\begin{minipage}{0.1\textwidth}\centering loss \end{minipage}}
% \end{overpic}
% \caption{\tb{Method overview.} Given a grayscale image $\grayimg$ as input, our model starts with detecting the object bounding boxes ($\instnboxi$) using an off-the-shelf object detection model. We then crop out every detected instance $\instngray$ via $\instnboxi$ and use instance colorization network to colorize $\instngray$. However, as the instances' colors may not be compatible with respect to the predicted background colors, we propose to fuse all the instances' feature maps in every layer with the extracted full-image feature map using the proposed fusion module. We can thus obtain globally consistent colorization results $\predimg$. Our training process sequentially trains our full-image colorization network, and the instance colorization network, and the proposed fusion module.}
% \label{fig:overview}
% \end{figure*}

==> Figure/fig_training_process.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/images/training_process.png}
    \caption{\tb{Training process.} We start by training the texture generator $\styleGAN$ following the procedure of StyleGAN2-ada~\cite{Karras2020ada}.
    Next, we train the style encoder $\estyle$ with frozen texture generator $\styleGAN$, and finally the structure encoder $\egeo$ with frozen texture generator $\styleGAN$ and style encoder $\estyle$. }
    \label{fig:training_process}
\end{figure}

==> Figure/tbl_baseline_uncondition.tex <==
\begin{table}[!t]
    \caption{\tb{Quantitative evaluation under unconditional setting.}}
    \label{tab:baseline_uncondition}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cllllll}
        \toprule
        & \multicolumn{3}{c}{cars} & \multicolumn{3}{c}{faces} \\ 
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        \multirow{-2}{*}{Method} & FID$\downarrow$ & KID$\downarrow$ & GIQA$\uparrow$ & FID$\downarrow$ & KID$\downarrow$ & GIQA$\uparrow$\\
        \midrule
        Texture Fields~\cite{OechsleICCV2019} & 149.21 & 0.1156 & 3.8107 & 25.44 & 0.0344 & 6.6823\\
        LTG~\cite{rui2021LTG} & 87.06 & 0.0806 & 4.4394 & 20.08 & \tb{0.0203} & 6.7668\\
        Ours & \tb{66.73} & \tb{0.0652} & \tb{4.6276} & \tb{18.66} & 0.0212 & \tb{7.0326} \\ 
        \bottomrule
        \end{tabular}
    }
\end{table}

==> Figure/tbl_different_segmentation_class.tex <==
\begin{table}[!t]
    \caption{\tb{Quantitative Comparison with different class number of segmentation label.}}
    \label{tab:seg_num}
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{clllllll}
    \toprule
    & &  \multicolumn{3}{c}{mIoU($\%$)$\uparrow$} & \multicolumn{3}{c}{Pixel Accuracy($\%$)$\uparrow$} \\ 
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    \multirow{-2}{*}{Class Number} & \multirow{-2}{*}{FID$\downarrow$} & Front & Back & Side & Front & Back & Side\\
    \midrule
    10 & \tb{39.41} & \tb{74.28} & \tb{64.94} & \tb{69.31} & \tb{87.97} & \tb{82.58} & \tb{82.84} \\
    14 & 43.78 & 71.17 & 53.83 & 62.43 & 81.42 & 67.23 & 81.19 \\
    32 & 43.85 & 56.47 & 50.54 & 51.45 & 67.21 & 62.94 & 62.15 \\
    \bottomrule
    \end{tabular}
    % }
\end{table}


==> Figure/tbl_example.tex <==
\begin{table*}[!t]
    \caption{\tb{Quantitative evaluation on XXX.} We evaluate our method on ...}
    \label{tab:my_label}
    \centering
    % \resizebox{\textwidth}{!}{
        \begin{tabular}{lllll}
        \toprule
        & \multicolumn{2}{c}{Dataset 1} & \multicolumn{2}{c}{Dataset 2} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        \multirow{-2}{*}{Method} & 2D IoU & 3D IoU & 2D IoU & 3D IoU \\
        \midrule
        XXX~\etal~\cite{chen2019sports} & 0.8798 & 0.8612 & \tb{0.9933} & \tb{0.9912} \\
        Ours & \tb{0.9856} & \tb{0.9543} & 0.9817 & 0.9512 \\
        \bottomrule
        \end{tabular}
    % }
\end{table*}

==> Figure/tbl_two_style_code_encoder.tex <==
\begin{table}[!t]
    \caption{\tb{Quantitative comparison of view-consistency ablation.} The evaluation are tested on Cars dataset.}
    \label{tab:two_style_code_encoder}
    \centering
    % \resizebox{\linewidth}{!}{
        \begin{tabular}{cc}
        \toprule
        Method & FID$\downarrow$ \\
        \midrule
        LTG~\cite{rui2021LTG} & 149.82\\
        Ours with silhouette input & 42.86 \\ 
        Ours with segmentation input & \tb{39.41} \\ 
        \bottomrule
        \end{tabular}
    % }
\end{table}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sup_text.tex <==
\section{Dataset details}
In the main paper, we evaluate our method on two datasets: Cars and Faces. The details of the data processing are as follows:
\begin{itemize}
    \item \emph{Cars}: 
    We use the CompCars dataset~\cite{yang2015compcars}, which contains 32,028 car photographs with labeled bounding boxes and viewpoints, as our dataset. We randomly select 16,000 images for training, 2000 images for validation, and 2,000 images for test. For each image, we apply a cropping operation based on the labeled bounding boxes and generate segmentation map $\semanticmapset$ on the training set using DatasetGAN~\cite{zhang2021datasetgan}, a segmentation generation network based on StyleGAN~\cite{karras2019style}, and set the number of semantic labels to 10. 
    %
    As for testing, we randomly choose 32 3D car models from ShapeNet~\cite{shapenet2015} to evaluate our method accompanied with 8 randomly selected CompCars images as style image $\styleimg$ and render the results from 8 camera views during a testing time for each car model. We preprocess the ShapeNet car models with zero-centering and normalization, apply the view-based parameterization method with Pytorch3D~\cite{ravi2020pytorch3d}, and obtain six canonical view (front, back, left, right, top and bottom) UV maps $\uvmapset$. We then label the segmentation maps on these views on the test set.
    
    \item \emph{Faces}: 
    We use FFHQ~\cite{Karras_2019_CVPR} dataset, a large-scale real-world human photographs collection containing 70,000 images, as our dataset. We discard the photographs that contain multiple people, randomly choose 65,747 images for training, 64 images for validation, and 3,000 images for testing, and obtain 3D models by ~\cite{deng2019accurate}. We apply the view-based parameterization method with Pytorch3D~\cite{ravi2020pytorch3d} to get the front-view UV maps $\uvmapset$ and apply perspective projection of 3D model to derive the RGB images as the style images $\styleimg$. We then use a BiSeNet face-parsing network~\cite{zllrunning2019} to generate paired segmentation maps $\semanticmapset$ on the canonical view, and set the number of semantic labels to 9. We render the results from 3 camera views using 1 style image $\styleimg$ per 3D model for testing.
\end{itemize}

\section{Ablation study on the class number of segmentation labels.}
\input{Figure/tbl_different_segmentation_class}
\input{Figure/fig_segmentation_result}
In this experiment, we investigate the effect of varying the number of semantic labels used in our method on the cars dataset under the conditional setting, which uses a segmentation map to label the structural details of the input 3D shape.
%
We manually select three different numbers of semantic labels (10, 14, and 32) and retrain our model on these three settings.
%
The quantitative results are presented in \tabref{seg_num}. Surprisingly, we find that as the number of semantic labels increases, the performance of our network deteriorates.
%
This trend is also reflected in the visual quality of the generated textures, as shown in \figref{different_seg_num_result}.
%
We speculate that the lower performance of the 32-class labeling scheme is due to insufficient supervision for fine-grained class labels such as "rear bumper," "back door handle," and "back logo."
%
While we label the model's semantic class, we manually add more detailed classes into the segmentation map as the number of classes increased.
%
For instance, when we labeled headlights in the 10-class scheme, we do not differentiate between left and right headlights. However, in the 32-class labeling scheme, we divide the label of headlights into left and right headlights for more detailed labeling.
%
As a result, fine-grained class labels in the 32-class labeling scheme appeared much less frequently than the general class labels in the 10-class scheme. Therefore, all classes in the 10-class scheme obtained more supervision than the classes in the 32-class labeling scheme since we keep the same amount of training data across different class labeling schemes. 
%
This explains the lower performance of the 32-class labeling scheme compared to the 10-class labeling scheme.

\section{More Results Under Conditional Setting}

% We present more visual results that generated by our model under conditional setting on the car dataset. 
% %
% We show our results include textured models rendered from 10 input 3D models and 8 style images for each 3D model, under 7 randomly selected views with segmentation maps. The first column shows the input 3D model along with six-view segmentation maps. The second column displays the input style images, while the remaining columns depict the textured models under 7 random viewing angles.
% %
% The visual results indicate that CTGAN is capable of producing the texture maps which are view-consistent and similar with the style image, and contain lots of fine-grained structural details without any noticeable texture seam. 

We present additional visual results generated by our model under conditional setting on the car dataset~\cite{shapenet2015}. Our results showcase textured models created from 10 input 3D models and 8 style images for each 3D model, viewed from 7 randomly selected angles, accompanied by segmentation maps.
%
In the first column, we present the input 3D model alongside six-view segmentation maps. The second column displays the input style images, while the remaining columns illustrate rendering the textured models from 7 random viewing angles.
%
Our visual results demonstrate that CTGAN is capable of producing view-consistent texture maps that are similar to the style image and also display a wealth of fine-grained structural details without any noticeable texture seams.

\input{Figure/fig_sup_result}
